The Infrared Telescope Facility (IRTF) Spectral Library: Cool Stars

We present a 0.8 -5 micron spectral library of 210 cool stars observed at a resolving power of R = lambda / Delta lambda ~ 2000 with the medium-resolution infrared spectrograph, SpeX, at the 3.0 m NASA Infrared Telescope Facility (IRTF) on Mauna Kea, Hawaii. The stars have well established MK spectral classifications and are mostly restricted to near-solar metallicities. The sample contains the F, G, K, and M spectral types with luminosity classes between I and V, but also includes some AGB, carbon, and S stars. In contrast to some other spectral libraries, the continuum shape of the spectra are measured and preserved in the data reduction process. The spectra are absolutely flux calibrated using Two Micron All Sky Survey (2MASS) photometry. Potential uses of the library include studying the physics of cool stars, classifying and studying embedded young clusters and optically obscured regions of the Galaxy, evolutionary population synthesis to study unresolved stellar populations in optically-obscured regions of galaxies, and synthetic photometry. The library is available in digital form from the IRTF website.

==> color.tex <==
\begin{deluxetable}{llccccc}
\tablecolumns{7}
\tabletypesize{\scriptsize} 
\tablewidth{0pc}
\tablecaption{\label{tab:MKOColors}Synthetic WFCAM Colors}
\tablehead{
\colhead{Object} & 
\colhead{Spectral} & 
\colhead{$Z-Y$} &
\colhead{$Y-J$} &
\colhead{$J-H$} &
\colhead{$H-K$} &
\colhead{$K-L'$} \\


\colhead{} & 
\colhead{Type} & 
\colhead{(mag)} &
\colhead{(mag)} &
\colhead{(mag)} &
\colhead{(mag)} &
\colhead{(mag)} \\

\colhead{(1)} & 
\colhead{(2)} & 
\colhead{(3)} & 
\colhead{(4)} & 
\colhead{(5)} & 
\colhead{(6)} & 
\colhead{(7)}}
 
\startdata
 
HD 7927 & F0 Ia & $+$0.161 & $+$0.211 & $+$0.257 & $+$0.152 & $+$0.208 \\
HD 135153 & F0 Ib$-$II & $+$0.113 & $+$0.153 & $+$0.186 & $+$0.087 & $+$0.044 \\
HD 6130 & F0 II & $+$0.147 & $+$0.193 & $+$0.225 & $+$0.090 & $+$0.128 \\
HD 89025 & F0 IIIa & $+$0.052 & $+$0.147 & $+$0.161 & $+$0.033 & $+$0.058 \\
HD 27397 & F0 IV & $+$0.058 & $+$0.115 & $+$0.107 & $-$0.011 & $-$0.018 \\
HD 108519 & F0 V(n) & $+$0.043 & $+$0.116 & $+$0.144 & $+$0.044 & $+$0.018 \\
HD 173638 & F1 II & $+$0.187 & $+$0.200 & $+$0.222 & $+$0.083 & $+$0.088 \\
HD 213135 & F1 V & $+$0.045 & $+$0.162 & $+$0.175 & $+$0.021 & $+$0.028 \\
BD $+$38 2803 & F2 I & $+$0.106 & $+$0.257 & $+$0.304 & $+$0.085 & $+$0.096 \\
HD 182835 & F2 Ib & $+$0.158 & $+$0.196 & $+$0.214 & $+$0.073 & $\cdots$ \\
HD 13174 & F2 III$-$IV & $+$0.066 & $+$0.155 & $+$0.153 & $+$0.018 & $+$0.053 \\
HD 40535 & F2 III$-$IV & $+$0.079 & $+$0.173 & $+$0.185 & $+$0.046 & $+$0.065 \\
HD 164136 & F2 IV & $+$0.080 & $+$0.197 & $+$0.210 & $+$0.031 & $+$0.110 \\
HD 113139 & F2 V & $+$0.084 & $+$0.187 & $+$0.184 & $+$0.026 & $-$0.092 \\
HD 26015 & F3 V & $+$0.061 & $+$0.144 & $+$0.119 & $-$0.014 & $-$0.045 \\
HD 21770 & F4 III & $+$0.050 & $+$0.168 & $+$0.181 & $+$0.030 & $+$0.068 \\
HD 87822 & F4 V & $+$0.065 & $+$0.182 & $+$0.182 & $+$0.038 & $+$0.052 \\
HD 16232 & F4 V & $+$0.050 & $+$0.175 & $+$0.207 & $+$0.035 & $+$0.113 \\
HD 213306 & F5 Ib $-$ G1 Ib & $+$0.181 & $+$0.295 & $+$0.363 & $+$0.084 & $+$0.029 \\
HD 186155 & F5 II$-$III & $+$0.047 & $+$0.159 & $+$0.158 & $+$0.039 & $-$0.007 \\
HD 17918 & F5 III & $+$0.082 & $+$0.184 & $+$0.190 & $+$0.013 & $+$0.019 \\
HD 218804 & F5 V & $+$0.082 & $+$0.206 & $+$0.242 & $+$0.058 & $+$0.073 \\
HD 27524 & F5 V & $+$0.036 & $+$0.173 & $+$0.183 & $+$0.028 & $+$0.045 \\
HD 75555 & F5.5 III$-$IV & $+$0.088 & $+$0.210 & $+$0.212 & $+$0.046 & $\cdots$ \\
HD 51956 & F6 IbII & $+$0.144 & $+$0.280 & $+$0.312 & $+$0.083 & $+$0.003 \\
HD 160365 & F6 III$-$IV & $+$0.033 & $+$0.159 & $+$0.174 & $-$0.028 & $+$0.012 \\
HD 11443 & F6 IV & $+$0.065 & $+$0.184 & $+$0.243 & $+$0.088 & $-$0.009 \\
HD 215648 & F6 V & $+$0.072 & $+$0.212 & $+$0.230 & $+$0.037 & $\cdots$ \\
HD 201078 & F7 II & $+$0.099 & $+$0.201 & $+$0.231 & $+$0.081 & $\cdots$ \\
HD 124850 & F7 III & $+$0.093 & $+$0.222 & $+$0.241 & $+$0.032 & $\cdots$ \\
HD 126660 & F7 V & $+$0.055 & $+$0.194 & $+$0.217 & $+$0.061 & $+$0.042 \\
HD 190323 & F8 Ia & $+$0.174 & $+$0.262 & $+$0.278 & $+$0.074 & $+$0.067 \\
HD 220657 & F8 III & $+$0.119 & $+$0.278 & $+$0.328 & $+$0.111 & $+$0.122 \\
HD 111844 & F8 IV & $+$0.044 & $+$0.119 & $+$0.105 & $+$0.009 & $\cdots$ \\
HD 219623 & F8 V & $+$0.103 & $+$0.222 & $+$0.258 & $+$0.056 & $-$0.012 \\
HD 27383 & F8 V & $+$0.086 & $+$0.194 & $+$0.213 & $+$0.021 & $-$0.017 \\
HD 102870 & F8.5 IV$-$V & $+$0.076 & $+$0.220 & $+$0.251 & $+$0.043 & $+$0.033 \\
HD 176051 & F9 V & $+$0.089 & $+$0.254 & $+$0.324 & $+$0.054 & $-$0.037 \\
HD 165908 & F9 V & $+$0.036 & $+$0.189 & $+$0.235 & $+$0.062 & $+$0.058 \\
HD 114710 & F9.5 V & $+$0.060 & $+$0.194 & $+$0.198 & $-$0.006 & $+$0.025 \\
HD 185018 & G0 Ib$-$II & $+$0.173 & $+$0.303 & $+$0.364 & $+$0.085 & $+$0.007 \\
HD 6903 & G0 IIIa & $+$0.127 & $+$0.268 & $+$0.320 & $+$0.072 & $+$0.043 \\
HD 109358 & G0 V & $+$0.079 & $+$0.235 & $+$0.294 & $+$0.034 & $+$0.010 \\
HD 74395 & G1 Ib & $+$0.175 & $+$0.298 & $+$0.348 & $+$0.086 & $+$0.062 \\
HD 216219 & G1 II$-$III: Fe$-$1 CH0.5 & $+$0.096 & $+$0.232 & $+$0.274 & $+$0.054 & $+$0.061 \\
HD 21018 & G1 III:CH$-$1: & $+$0.175 & $+$0.305 & $+$0.353 & $+$0.102 & $+$0.066 \\
HD 10307 & G1 V & $+$0.092 & $+$0.233 & $+$0.281 & $+$0.037 & $+$0.029 \\
HD 95128 & G1$-$ V Fe$-$0.5 & $+$0.110 & $+$0.253 & $+$0.273 & $+$0.045 & $\cdots$ \\
HD 20619 & G1.5 V & $+$0.122 & $+$0.278 & $+$0.344 & $+$0.077 & $+$0.053 \\
HD 42454 & G2 Ib & $+$0.264 & $+$0.369 & $+$0.415 & $+$0.122 & $\cdots$ \\
HD 39949 & G2 Ib & $+$0.250 & $+$0.361 & $+$0.424 & $+$0.118 & $\cdots$ \\
HD 3421 & G2 Ib$-$II & $+$0.175 & $+$0.289 & $+$0.370 & $+$0.075 & $+$0.076 \\
HD 219477 & G2 II$-$III & $+$0.125 & $+$0.269 & $+$0.320 & $+$0.065 & $\cdots$ \\
HD 126868 & G2 IV & $+$0.107 & $+$0.246 & $+$0.318 & $+$0.074 & $+$0.090 \\
HD 76151 & G2 V & $+$0.100 & $+$0.250 & $+$0.304 & $+$0.083 & $+$0.044 \\
HD 192713 & G3 Ib$-$II & $+$0.226 & $+$0.345 & $+$0.422 & $+$0.108 & $+$0.085 \\
HD 176123 & G3 II & $+$0.211 & $+$0.345 & $+$0.410 & $+$0.089 & $+$0.098 \\
HD 88639 & G3 III Fe$-$1 & $+$0.169 & $+$0.318 & $+$0.394 & $+$0.069 & $+$0.112 \\
HD 10697 & G3 V & $+$0.140 & $+$0.279 & $+$0.331 & $+$0.088 & $+$0.082 \\
HD 179821 & G4 O$-$Ia & $+$0.301 & $+$0.368 & $+$0.394 & $+$0.249 & $+$0.239 \\
HD 6474 & G4 Ia & $+$0.408 & $+$0.472 & $+$0.492 & $+$0.235 & $+$0.217 \\
HD 94481 & G4 III & $+$0.163 & $+$0.311 & $+$0.402 & $+$0.083 & $\cdots$ \\
HD 108477 & G4 III & $+$0.181 & $+$0.319 & $+$0.399 & $+$0.099 & $+$0.096 \\
HD 214850 & G4 V & $+$0.103 & $+$0.273 & $+$0.395 & $+$0.108 & $+$0.059 \\
HD 190113 & G5 Ib & $+$0.300 & $+$0.428 & $+$0.531 & $+$0.150 & $+$0.133 \\
HD 18474 & G5 III: CN$-$3 CH$-$2 & $+$0.162 & $+$0.313 & $+$0.420 & $+$0.045 & $+$0.074 \\
HD 193896 & G5 IIIa & $+$0.229 & $+$0.363 & $+$0.449 & $+$0.124 & $\cdots$ \\
HD 165185 & G5 V & $+$0.056 & $+$0.218 & $+$0.259 & $+$0.055 & $-$0.014 \\
HD 161664 & G6 Ib H$_\delta$1 & $+$0.397 & $+$0.490 & $+$0.565 & $+$0.179 & $+$0.185 \\
HD 202314 & G6 Ib$-$IIa Ca1 Ba 0.5 & $+$0.239 & $+$0.357 & $+$0.451 & $+$0.162 & $+$0.161 \\
HD 58367 & G6 II & $+$0.203 & $+$0.335 & $+$0.434 & $+$0.099 & $+$0.131 \\
HD 27277 & G6 III & $+$0.238 & $+$0.354 & $+$0.420 & $+$0.094 & $+$0.093 \\
HD 20618 & G6 IV & $+$0.181 & $+$0.331 & $+$0.439 & $+$0.098 & $+$0.093 \\
HD 115617 & G6.5 V & $+$0.086 & $+$0.232 & $+$0.285 & $+$0.020 & $-$0.031 \\
HD 333385 & G7 Ia & $+$0.557 & $+$0.562 & $+$0.545 & $+$0.306 & $+$0.594 \\
HD 182694 & G7 IIIa & $+$0.157 & $+$0.318 & $+$0.408 & $+$0.107 & $+$0.044 \\
HD 114946 & G7 IV$-$V & $+$0.165 & $+$0.328 & $+$0.451 & $+$0.094 & $+$0.120 \\
HD 208606 & G8 Ib & $+$0.411 & $+$0.494 & $+$0.596 & $+$0.202 & $+$0.099 \\
HD 25877 & G8 IIa & $+$0.206 & $+$0.328 & $+$0.400 & $+$0.076 & $+$0.081 \\
HD 122563 & G8: II:Fe $-$5 & $+$0.204 & $+$0.374 & $+$0.532 & $+$0.112 & $+$0.051 \\
HD 104979 & G8 IIIa CN$-$1 Ba1 CH1 & $+$0.184 & $+$0.337 & $+$0.486 & $+$0.098 & $+$0.132 \\
HD 135722 & G8 III  Fe$-$1 & $+$0.185 & $+$0.343 & $+$0.495 & $+$0.120 & $-$0.006 \\
HD 16139 & G8.5 IIIa Fe$-$0.5 & $+$0.226 & $+$0.357 & $+$0.458 & $+$0.130 & $+$0.078 \\
HD 101501 & G8 V & $+$0.133 & $+$0.270 & $+$0.332 & $+$0.062 & $+$0.012 \\
HD 75732 & G8 V & $+$0.148 & $+$0.290 & $+$0.364 & $+$0.103 & $+$0.071 \\
HD 170820 & G9 II CN1 Hd1 & $+$0.455 & $+$0.541 & $+$0.613 & $+$0.221 & $+$0.157 \\
HD 222093 & G9 III & $+$0.202 & $+$0.367 & $+$0.503 & $+$0.102 & $+$0.070 \\
HD 165782 & K0 Ia & $+$0.584 & $+$0.579 & $+$0.551 & $+$0.289 & $\cdots$ \\
HD 44391 & K0 Ib & $+$0.303 & $+$0.429 & $+$0.540 & $+$0.168 & $+$0.117 \\
HD 179870 & K0 II & $+$0.274 & $+$0.386 & $+$0.439 & $+$0.048 & $-$0.016 \\
HD 100006 & K0 III & $+$0.235 & $+$0.380 & $+$0.531 & $+$0.104 & $+$0.109 \\
HD 145675 & K0 V & $+$0.140 & $+$0.290 & $+$0.340 & $+$0.058 & $-$0.017 \\
HD 164349 & K0.5 IIb & $+$0.250 & $+$0.371 & $+$0.470 & $+$0.074 & $\cdots$ \\
HD 9852 & K0.5 IIIa CN1 & $+$0.348 & $+$0.472 & $+$0.601 & $+$0.153 & $+$0.092 \\
HD 63302 & K1 Ia$-$Iab & $+$0.383 & $+$0.486 & $+$0.584 & $+$0.215 & $+$0.205 \\
HD 36134 & K1 III$-$ & $+$0.229 & $+$0.390 & $+$0.538 & $+$0.097 & $+$0.097 \\
HD 91810 & K1 IIIb CN1.5 Ca1 & $+$0.263 & $+$0.401 & $+$0.528 & $+$0.134 & $+$0.138 \\
HD 25975 & K1 III & $+$0.149 & $+$0.312 & $+$0.424 & $+$0.075 & $+$0.042 \\
HD 165438 & K1 IV & $+$0.194 & $+$0.350 & $+$0.454 & $+$0.098 & $\cdots$ \\
HD 142091 & K1 IVa & $+$0.199 & $+$0.341 & $+$0.454 & $+$0.084 & $\cdots$ \\
HD 10476 & K1 V & $+$0.147 & $+$0.317 & $+$0.405 & $+$0.095 & $+$0.031 \\
HD 124897 & K1.5 III Fe$-$0.5 & $+$0.246 & $+$0.420 & $+$0.651 & $+$0.127 & $+$0.076 \\
HD 212466 & K2 O$-$Ia & $+$0.635 & $+$0.619 & $+$0.623 & $+$0.399 & $+$0.302 \\
HD 2901 & K2 III Fe$-$0.5 & $+$0.284 & $+$0.436 & $+$0.605 & $+$0.096 & $+$0.125 \\
HD 132935 & K2 III & $+$0.298 & $+$0.462 & $+$0.661 & $+$0.164 & $+$0.127 \\
HD 137759 & K2 III & $+$0.264 & $+$0.420 & $+$0.564 & $+$0.140 & $\cdots$ \\
HD 3765 & K2 V & $+$0.166 & $+$0.330 & $+$0.420 & $+$0.080 & $+$0.049 \\
HD 23082 & K2.5 II CN0.5 & $+$0.457 & $+$0.550 & $+$0.699 & $+$0.204 & $+$0.199 \\
HD 187238 & K3 Iab$-$Ib & $+$0.553 & $+$0.597 & $+$0.729 & $+$0.227 & $+$0.254 \\
HD 221246 & K3 III & $+$0.332 & $+$0.472 & $+$0.658 & $+$0.144 & $+$0.178 \\
HD 178208 & K3 III & $+$0.315 & $+$0.453 & $+$0.589 & $+$0.142 & $\cdots$ \\
HD 35620 & K3.5 III CN2 & $+$0.326 & $+$0.459 & $+$0.618 & $+$0.170 & $+$0.061 \\
HD 219134 & K3 V & $+$0.245 & $+$0.384 & $+$0.512 & $+$0.117 & $+$0.086 \\
HD 16068 & K3.5 II$-$III Ca1 & $+$0.440 & $+$0.538 & $+$0.706 & $+$0.173 & $+$0.223 \\
HD 99998 & K3.5 III Fe$-$1 & $+$0.347 & $+$0.526 & $+$0.744 & $+$0.195 & $+$0.144 \\
HD 185622 & K4 Ib & $+$0.546 & $+$0.622 & $+$0.810 & $+$0.298 & $\cdots$ \\
HD 201065 & K4 Ib$-$II & $+$0.444 & $+$0.563 & $+$0.753 & $+$0.223 & $+$0.181 \\
HD 207991 & K4$-$ III & $+$0.384 & $+$0.533 & $+$0.771 & $+$0.202 & $+$0.058 \\
HD 114960 & K4 III CN0.5 & $+$0.314 & $+$0.443 & $+$0.616 & $+$0.153 & $+$0.072 \\
HD 45977 & K4 V & $+$0.192 & $+$0.351 & $+$0.480 & $+$0.105 & $\cdots$ \\
HD 216946 & K5 Ib & $+$0.562 & $+$0.660 & $+$0.862 & $+$0.318 & $+$0.211 \\
HD 181596 & K5 III & $+$0.385 & $+$0.525 & $+$0.727 & $+$0.196 & $+$0.154 \\
HD 36003 & K5 V & $+$0.221 & $+$0.388 & $+$0.559 & $+$0.125 & $+$0.021 \\
HD 120477 & K5.5 III & $+$0.372 & $+$0.521 & $+$0.736 & $+$0.211 & $+$0.164 \\
HD 3346 & K6 III & $+$0.364 & $+$0.529 & $+$0.772 & $+$0.230 & $\cdots$ \\
HD 181475 & K7 IIa & $+$0.574 & $+$0.660 & $+$0.853 & $+$0.308 & $\cdots$ \\
HD 194193 & K7 III & $+$0.401 & $+$0.549 & $+$0.811 & $+$0.225 & $+$0.106 \\
HD 237903 & K7 V & $+$0.271 & $+$0.430 & $+$0.608 & $+$0.134 & $+$0.112 \\
HD 201092 & K7 V & $+$0.212 & $+$0.374 & $+$0.554 & $+$0.151 & $\cdots$ \\
HD 213893 & M0 IIIb & $+$0.390 & $+$0.526 & $+$0.759 & $+$0.200 & $+$0.086 \\
HD 19305 & M0 V & $+$0.287 & $+$0.437 & $+$0.632 & $+$0.182 & $+$0.074 \\
HD 236697 & M0.5 Ib & $+$0.579 & $+$0.673 & $+$0.839 & $+$0.304 & $+$0.273 \\
HD 209290 & M0.5 V & $+$0.336 & $+$0.476 & $+$0.629 & $+$0.217 & $+$0.195 \\
HD 339034 & M1 Ia & $+$0.983 & $+$0.906 & $+$0.922 & $+$0.491 & $+$0.516 \\
HD 14404 & M1$-$ Iab$-$Ib & $+$0.613 & $+$0.666 & $+$0.804 & $+$0.303 & $+$0.337 \\
HD 39801 & M1$-$M2 Ia$-$Iab & $+$0.474 & $+$0.523 & $+$0.658 & $+$0.111 & $+$0.616 \\
HD 204724 & M1$+$ III & $+$0.394 & $+$0.491 & $+$0.713 & $+$0.253 & $+$0.085 \\
HD 42581 & M1 V & $+$0.332 & $+$0.456 & $+$0.606 & $+$0.210 & $+$0.199 \\
HD 35601 & M1.5 Iab$-$Ib & $+$0.638 & $+$0.717 & $+$0.863 & $+$0.362 & $+$0.253 \\
BD $+$60 265 & M1.5 Ib & $+$0.655 & $+$0.727 & $+$0.870 & $+$0.388 & $+$0.355 \\
HD 36395 & M1.5 V & $+$0.360 & $+$0.487 & $+$0.675 & $+$0.203 & $+$0.104 \\
HD 206936 & M2$-$ Ia & $+$0.603 & $+$0.643 & $+$0.755 & $+$0.409 & $+$0.462 \\
HD 10465 & M2 Ib & $+$0.528 & $+$0.599 & $+$0.756 & $+$0.278 & $+$0.163 \\
HD 23475 & M2$+$ IIab & $+$0.473 & $+$0.571 & $+$0.813 & $+$0.256 & $\cdots$ \\
HD 120052 & M2 III & $+$0.427 & $+$0.589 & $+$0.841 & $+$0.271 & $+$0.087 \\
HD 95735 & M2 V & $+$0.339 & $+$0.460 & $+$0.512 & $+$0.216 & $+$0.310 \\
Gl 806 & M2 V & $+$0.340 & $+$0.458 & $+$0.562 & $+$0.187 & $\cdots$ \\
HD 219734 & M2.5 III Ba0.5 & $+$0.446 & $+$0.570 & $+$0.809 & $+$0.245 & $+$0.084 \\
Gl 381 & M2.5 V & $+$0.398 & $+$0.500 & $+$0.550 & $+$0.242 & $+$0.263 \\
Gl 581 & M2.5 V & $+$0.406 & $+$0.486 & $+$0.523 & $+$0.280 & $+$0.301 \\
RW Cyg & M3$-$M4 Ia$-$Iab & $+$0.839 & $+$0.820 & $+$0.982 & $+$0.448 & $+$0.356 \\
CD $-$31 4916 & M3 Iab$-$Ia & $+$0.637 & $+$0.700 & $+$0.851 & $+$0.342 & $+$0.395 \\
HD 14488 & M3$+$ Iab & $+$0.727 & $+$0.724 & $+$0.949 & $+$0.495 & $+$0.331 \\
HD 14469 & M3$-$M4 Iab & $+$0.705 & $+$0.679 & $+$0.805 & $+$0.367 & $+$0.284 \\
HD 40239 & M3 II & $+$0.530 & $+$0.626 & $+$0.862 & $+$0.300 & $+$0.212 \\
HD 39045 & M3 III & $+$0.466 & $+$0.593 & $+$0.829 & $+$0.267 & $+$0.172 \\
Gl 388 & M3 V & $+$0.421 & $+$0.504 & $+$0.559 & $+$0.237 & $+$0.249 \\
Gl 815A & M3 Ve & $+$0.322 & $+$0.442 & $+$0.533 & $+$0.188 & $\cdots$ \\
HD 28487 & M3.5 III & $+$0.550 & $+$0.623 & $+$0.875 & $+$0.292 & $+$0.165 \\
Gl 273 & M3.5 V & $+$0.476 & $+$0.526 & $+$0.515 & $+$0.284 & $+$0.311 \\
HD 19058 & M4 II & $+$0.551 & $+$0.603 & $+$0.878 & $+$0.297 & $+$0.075 \\
HD 214665 & M4$+$ III & $+$0.694 & $+$0.726 & $+$0.954 & $+$0.335 & $+$0.031 \\
HD 4408 & M4 IIIa & $+$0.521 & $+$0.598 & $+$0.856 & $+$0.297 & $+$0.027 \\
HD 27598 & M4$-$ III & $+$0.500 & $+$0.572 & $+$0.820 & $+$0.272 & $+$0.165 \\
Gl 213 & M4 V & $+$0.500 & $+$0.523 & $+$0.464 & $+$0.281 & $+$0.368 \\
Gl 299 & M4 V & $+$0.485 & $+$0.525 & $+$0.411 & $+$0.310 & $+$0.464 \\
Gl 630.1A & M4 Ve & $+$0.505 & $+$0.544 & $+$0.450 & $+$0.262 & $+$0.345 \\
HD 204585 & M4.5 IIIa & $+$0.621 & $+$0.590 & $+$0.780 & $+$0.234 & $\cdots$ \\
Gl 268AB & M4.5 V & $+$0.552 & $+$0.570 & $+$0.535 & $+$0.311 & $+$0.392 \\
HD 156014 & M5 Ib$-$II & $+$0.647 & $+$0.517 & $+$0.614 & $+$0.097 & $+$0.188 \\
HD 175865 & M5 III & $+$0.648 & $+$0.601 & $+$0.798 & $+$0.229 & $\cdots$ \\
Gl 51 & M5 V & $+$0.601 & $+$0.612 & $+$0.538 & $+$0.331 & $+$0.335 \\
Gl 866ABC & M5 V & $+$0.727 & $+$0.677 & $+$0.556 & $+$0.370 & $+$0.457 \\
HD 94705 & M5.5 III & $+$0.755 & $+$0.643 & $+$0.827 & $+$0.333 & $+$0.175 \\
HD 196610 & M6 III & $+$0.851 & $+$0.629 & $+$0.789 & $+$0.284 & $-$0.091 \\
HD 18191 & M6$-$ III & $+$0.794 & $+$0.669 & $+$0.870 & $+$0.319 & $-$0.012 \\
Gl 406 & M6 V & $+$0.824 & $+$0.719 & $+$0.563 & $+$0.415 & $+$0.513 \\
GJ 1111 & M6.5 V & $+$0.841 & $+$0.726 & $+$0.524 & $+$0.422 & $+$0.516 \\
HD 14386 & M5e$-$M9e III & $+$1.213 & $+$0.654 & $+$0.519 & $+$0.519 & $+$0.600 \\
HD 108849 & M7$-$ III: & $+$1.151 & $+$0.811 & $+$0.814 & $+$0.414 & $+$0.204 \\
HD 207076 & M7$-$ III: & $+$1.007 & $+$0.649 & $+$0.697 & $+$0.282 & $+$0.498 \\
Gl 644C & M7 V & $+$0.861 & $+$0.745 & $+$0.505 & $+$0.438 & $+$0.544 \\
MY Cep & M7$-$M7.5 I & $+$1.469 & $+$1.246 & $+$1.315 & $+$0.814 & $+$0.919 \\
HD 69243 & M6e$-$M9e III & $+$1.533 & $+$1.258 & $+$0.738 & $+$0.611 & $+$0.707 \\
BRI B2339$-$0447 & M7$-$8 III & $+$0.701 & $+$0.589 & $+$0.819 & $+$0.498 & $+$0.590 \\
IRAS 01037$+$1219 & M8 III & $+$2.767 & $+$2.545 & $+$2.244 & $+$1.787 & $+$2.288 \\
Gl 752B & M8 V & $+$1.039 & $+$0.824 & $+$0.543 & $+$0.487 & $+$0.590 \\
LP 412$-$31 & M8 V & $+$1.030 & $+$0.893 & $+$0.630 & $+$0.486 & $+$0.612 \\
IRAS 21284$-$0747 & M8$-$9 III & $+$1.536 & $+$1.092 & $+$0.693 & $+$0.673 & $+$0.822 \\
IRAS 14436$-$0703 & M8$-$9 III & $+$1.437 & $+$0.925 & $+$0.575 & $+$0.601 & $\cdots$ \\
IRAS 14303$-$1042 & M8$-$9 III & $+$1.251 & $+$0.761 & $+$0.586 & $+$0.657 & $\cdots$ \\
IRAS 15060$+$0947 & M9 III & $+$1.350 & $+$1.011 & $+$1.162 & $+$1.206 & $\cdots$ \\
BRI B1219$-$1336 & M9 III & $+$1.273 & $+$0.843 & $+$0.602 & $+$0.577 & $\cdots$ \\
DENIS$-$P J104814.7$-$395606.1 & M9 V & $+$1.101 & $+$0.879 & $+$0.505 & $+$0.481 & $+$0.681 \\
LP 944$-$20 & M9 V & $+$1.253 & $+$0.994 & $+$0.592 & $+$0.536 & $+$0.750 \\
LHS 2065 & M9 V & $+$1.209 & $+$1.004 & $+$0.698 & $+$0.569 & $\cdots$ \\
LHS 2924 & M9 V & $+$1.209 & $+$0.999 & $+$0.657 & $+$0.536 & $\cdots$ \\
BRI B0021$-$0214 & M9.5 V & $+$1.244 & $+$1.085 & $+$0.698 & $+$0.591 & $+$0.661 \\
IRAS 14086$-$0703 & M10$+$ III & $+$2.219 & $+$2.128 & $+$1.885 & $+$2.054 & $\cdots$ \\
HD 142143 & M6.5S & $+$0.975 & $+$0.787 & $+$0.876 & $+$0.431 & $+$0.256 \\
BD $+$44 2267 & S2.5 Zr 2 & $+$0.456 & $+$0.566 & $+$0.762 & $+$0.242 & $+$0.245 \\
HD 64332 & S4.5 Zr 2 Ti 4 & $+$0.488 & $+$0.596 & $+$0.817 & $+$0.285 & $+$0.219 \\
HD 44544 & SC5.5 Zr 0.5 & $+$0.812 & $+$0.823 & $+$1.031 & $+$0.414 & $+$0.494 \\
HD 62164 & S5$-$S6 Zr 3$-$4 Ti 0 & $+$0.661 & $+$0.742 & $+$0.972 & $+$0.409 & $+$0.315 \\
HD 76846 & C$-$R2$+$ IIIa: C2 2.5 & $+$0.374 & $+$0.370 & $+$0.475 & $+$0.175 & $+$0.240 \\
HD 31996 & C7,6e(N4) & $+$0.649 & $+$0.947 & $+$1.279 & $+$1.187 & $+$1.152 \\
HD 44984 & C$-$N4 C2 3.5 & $+$0.638 & $+$0.580 & $+$0.901 & $+$0.437 & $+$0.403 \\
HD 76221 & C$-$N 4.5 C2 5.5 MS 3 & $+$0.620 & $+$0.657 & $+$1.008 & $+$0.645 & $+$0.593 \\
HD 92055 & C$-$N4.5 C2 4.5 & $+$0.651 & $+$0.655 & $+$0.989 & $+$0.480 & $+$0.493 \\
HD 70138 & C$-$J4.5 IIIa C2 6 j 6 & $+$0.657 & $+$0.482 & $+$0.893 & $+$0.491 & $+$0.622 \\
HD 48664 & C$-$N5 C2 6 & $+$0.745 & $+$0.725 & $+$1.067 & $+$0.646 & $+$0.643 \\
HD 57160 & C$-$J5$-$ C2 5$-$ j4 & $+$0.627 & $+$0.646 & $+$0.999 & $+$0.582 & $+$0.625 \\
\enddata
\end{deluxetable}

